A rotation-driven pulsar radio emission mechanism

We propose and discuss an alternative pulsar radio emission mechanism that relies on rotation-driven plasma oscillations, rather than on a beam-driven instability, and suggest that it may be the generic radio emission mechanism for pulsars. We identify these oscillations as superluminal longitudinal waves in the pulsar plasma, and point out that these waves can escape directly in the O~mode. We argue that the frequency of the oscillations is $\omega_0\approx\omega_{\rm p}(2\langle\gamma\rangle)^{1/2}/\gamma_{\rm s}$, where $\gamma_{\rm s}$ is the Lorentz factor of bulk streaming motion and $\langle\gamma\rangle$ is the mean Lorentz factor in the rest frame of the plasma. The dependence of the plasma frequency $\omega_{\rm p}$ on radial distance implies a specific frequency-to-radius mapping, $\omega_0\propto r^{-3/2}$. Escape of the energy in these oscillations is possible if they are generated in overdense, field-aligned regions that we call fibers; the wave energy is initially refracted into underdense regions between the fibers, which act as ducts. Some implications of the model for the interpretation of pulsar radio emission are discussed.

==> fig1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{018}[tc][tc]{\matlabtextA $ z $}%
\psfrag{019}[bc][bc]{\matlabtextA $ z' $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 4$}%
\psfrag{001}[ct][ct]{\matlabtextB $\matlabfragNegXTick 3$}%
\psfrag{002}[ct][ct]{\matlabtextB $\matlabfragNegXTick 2$}%
\psfrag{003}[ct][ct]{\matlabtextB $\matlabfragNegXTick 1$}%
\psfrag{004}[ct][ct]{\matlabtextB $0$}%
\psfrag{005}[ct][ct]{\matlabtextB $1$}%
\psfrag{006}[ct][ct]{\matlabtextB $2$}%
\psfrag{007}[ct][ct]{\matlabtextB $3$}%
\psfrag{008}[ct][ct]{\matlabtextB $4$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextB $-4$}%
\psfrag{010}[rc][rc]{\matlabtextB $-3$}%
\psfrag{011}[rc][rc]{\matlabtextB $-2$}%
\psfrag{012}[rc][rc]{\matlabtextB $-1$}%
\psfrag{013}[rc][rc]{\matlabtextB $0$}%
\psfrag{014}[rc][rc]{\matlabtextB $1$}%
\psfrag{015}[rc][rc]{\matlabtextB $2$}%
\psfrag{016}[rc][rc]{\matlabtextB $3$}%
\psfrag{017}[rc][rc]{\matlabtextB $4$}%
%
%% </ytick>

==> fig2a.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11.00}{11.00}\selectfont\strut}%
\psfrag{008}[tc][tc]{\matlabtextA $ \gamma_{\rm s} $}%
\psfrag{009}[bc][bc]{\matlabtextA $ r/R_* $}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10.00}{10.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $10^{0}$}%
\psfrag{001}[ct][ct]{\matlabtextB $10^{1}$}%
\psfrag{002}[ct][ct]{\matlabtextB $10^{2}$}%
\psfrag{003}[ct][ct]{\matlabtextB $10^{3}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{005}[rc][rc]{\matlabtextB $10^{1}$}%
\psfrag{006}[rc][rc]{\matlabtextB $10^{2}$}%
\psfrag{007}[rc][rc]{\matlabtextB $10^{3}$}%
%
%% </ytick>

==> fig2b.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11.00}{11.00}\selectfont\strut}%
\psfrag{008}[tc][tc]{\matlabtextA $ \gamma_{\rm s} $}%
\psfrag{009}[bc][bc]{\matlabtextA $ r/R_* $}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10.00}{10.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $10^{0}$}%
\psfrag{001}[ct][ct]{\matlabtextB $10^{1}$}%
\psfrag{002}[ct][ct]{\matlabtextB $10^{2}$}%
\psfrag{003}[ct][ct]{\matlabtextB $10^{3}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{005}[rc][rc]{\matlabtextB $10^{1}$}%
\psfrag{006}[rc][rc]{\matlabtextB $10^{2}$}%
\psfrag{007}[rc][rc]{\matlabtextB $10^{3}$}%
%
%% </ytick>

==> fig2c.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11.00}{11.00}\selectfont\strut}%
\psfrag{008}[tc][tc]{\matlabtextA $ \gamma_{\rm s} $}%
\psfrag{009}[bc][bc]{\matlabtextA $ r/R_* $}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10.00}{10.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $10^{0}$}%
\psfrag{001}[ct][ct]{\matlabtextB $10^{1}$}%
\psfrag{002}[ct][ct]{\matlabtextB $10^{2}$}%
\psfrag{003}[ct][ct]{\matlabtextB $10^{3}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{005}[rc][rc]{\matlabtextB $10^{1}$}%
\psfrag{006}[rc][rc]{\matlabtextB $10^{2}$}%
\psfrag{007}[rc][rc]{\matlabtextB $10^{3}$}%
%
%% </ytick>
